ROBUST: 221 Bugs in the Robot Operating System

As robotic systems such as autonomous cars and delivery drones assume greater roles and responsibilities within society, the likelihood and impact of catastrophic software failure within those systems is increased.To aid researchers in the development of new methods to measure and assure the safety and quality of robotics software, we systematically curated a dataset of 221 bugs across 7 popular and diverse software systems implemented via the Robot Operating System (ROS). We produce historically accurate recreations of each of the 221 defective software versions in the form of Docker images, and use a grounded theory approach to examine and categorize their corresponding faults, failures, and fixes. Finally, we reflect on the implications of our findings and outline future research directions for the community.

==> e964bbb.tex <==
%YAML 1.1
---
id: e964bbb
title: Calculation Error Inverts Turning Direction
description: "Due to an error in velocity calculations, when Kobuki was issued a 
  very low negative linear speed (slow backwards movement), it would also 
  inadvertently invert its turning direction. That is, if it was supposed to move 
  backwards while turning left, it would move backwards and turn right instead."
^\textbf{CWE}^: 
  id: 242
  description: Incorrect Calculation
keywords: ['differential drive', 'velocity', 'driver', 'movement']
system: kobuki
failure-codes: [ 'PROGRAMMING:CALCULATIONS' ]
fault-codes: [ 'SYSTEM:UNINTENDED-BEHAVIOUR', 'SYSTEM:MOTION' ]
bug:
  phase: runtime
  architectural-location: application-specific code
  task: locomotion
  package: yujinrobot/kobuki/kobuki_driver
  detected-by: developer
  reported-by: contributor
  issue: https://github.com/yujinrobot/kobuki/issues/227
  time-reported: 2013-02-22T09:09:21Z
fix:
  ^\textbf{commits}^:
    - repo: https://github.com/yujinrobot/kobuki
      hash: e964bbb8700fb1a9b95c0cfe5a44d43321294d4f
  pull-request: null
  fix-in: ['kobuki_driver/src/driver/diff_drive.cpp']
  languages: ['C++']
  time: 2013-02-25 (09:31)

